Fine-tuning Vision Classifiers On A Budget

Fine-tuning modern computer vision models requires accurately labeled data for which the ground truth may not exist, but a set of multiple labels can be obtained from labelers of variable accuracy. We tie the notion of label quality to confidence in labeler accuracy and show that, when prior estimates of labeler accuracy are available, using a simple naive-Bayes model to estimate the true labels allows us to label more data on a fixed budget without compromising label or fine-tuning quality. We present experiments on a dataset of industrial images that demonstrates that our method, called Ground Truth Extension (GTX), enables fine-tuning ML models using fewer human labels.

==> figures/uncertainty_sampling_bar_graph.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{figures/uncertainty_sampling_figures/exp1_small_cohort_bar_graphs.png}
    \caption{Distribution of Labels per Example for Uncertainty Sampling}
    \label{fig:u_s_experiment_bar_graphs}
\end{figure}


==> tables/finetuning.tex <==

\begin{table}
\label{tab:finetuning_high_quality_cohort}
\centering
\scriptsize{
% \begin{tabular}{ l c c c c c c c c c c  c c c c c c c c c c c c  }
%  \toprule
%         & \multicolumn{11}{c}{Balanced accuracy}    & \multicolumn{11}{c}{F1 score}     \\
%         \cmidrule(r){2-12} \cmidrule(r){13-23}
% Method  & a & b & c & d & e & f & g & h & k & l & ave & a & b & c & d & e & f & g & h & k & l & ave \\
% \midrule
% MV          & & & & & & & & & & & & & & & & & & & & & & \\
% WMV         & & & & & & & & & & & & & & & & & & & & & & \\
% SV          & & & & & & & & & & & & & & & & & & & & & & \\
% GTX (ours)  & & & & & & & & & & & & & & & & & & & & & & \\
%  \bottomrule
% \end{tabular}
\begin{tabular}{ l c c c c c c c c c c c c c c c }
\toprule
   & \multicolumn{5}{c}{Num images labeled} & \multicolumn{5}{c}{Balanced error} & \multicolumn{5}{c}{ECE} \\
        \cmidrule(r){2-6} \cmidrule(r){7-11} \cmidrule(r){12-16}
   & 250 & 500 & 1000 & 1500 & 4000 & 250 & 500 & 1000 & 1500 & 4000 & 250 & 500 & 1000 & 1500 & 4000 \\
 \midrule
 MV     & & & & \\
 WMV    & & & & \\
 SV     & & & & \\
 GTX    & 129.4 & 259.6 & 518.0 & 736.2 & 840.0 & 4.2\% & 2.0\% & 1.8\% & 1.5\% & 1.9\% & 8.1\% & 4.5\% & 5.1\% & 5.4\% & 4.2\% \\
 \bottomrule
 \end{tabular}
 }
 \caption{Performance of fine-tuned EfficientNet-b0 on the binary image classification task labeled with different methods and a high-quality labeler cohort.}

\end{table}

